Policy Optimization for Unknown Systems using Differentiable Model Predictive Control

Model-based policy optimization often struggles with inaccurate system dynamics models, leading to suboptimal closed-loop performance. This challenge is especially evident in Model Predictive Control (MPC) policies, which rely on the model for real-time trajectory planning and optimization. We introduce a novel policy optimization framework for MPC-based policies combining differentiable optimization with zeroth-order optimization. Our method combines model-based and model-free gradient estimation approaches, achieving faster transient performance compared to fully data-driven approaches while maintaining convergence guarantees, even under model uncertainty. We demonstrate the effectiveness of the proposed approach on a nonlinear control task involving a 12-dimensional quadcopter model.

==> Sources/header.tex <==
% References
\usepackage{csquotes}
\usepackage[english]{babel}

% Algorithms
\RequirePackage{algorithm,algpseudocode}
\algnewcommand\algorithmicinit{\textbf{Init:}}
\algnewcommand\Init{\item[\algorithmicinit]}
\algnewcommand\algorithmicinput{\textbf{Input:}}
\algnewcommand\Input{\item[\algorithmicinput]}

% tables
\usepackage{booktabs}
\usepackage{multirow}

% Math packages
\usepackage{dsfont}
\usepackage{mathrsfs}
\usepackage{amsfonts}   
\usepackage{mathtools}

\usepackage[hang,flushmargin]{footmisc}

% Fonts
\let\Bbbk\relax
\usepackage{times}
\usepackage[cmintegrals,cmbraces,varbb]{newtxmath} % Math font
\usepackage[cal=cm,bb=ams]{mathalpha} % Improve calligraphic and bb math
\renewcommand{\ttfamily}{\fontencoding{T1}\fontfamily{lmtt}\selectfont}

% Additional math options
\usepackage{xspace}

% theorems
\newtheorem{assumption}{Assumption}

% Math commands
\DeclareMathOperator*{\argmin}{arg\,min}

% Project-specific definitions
\newcommand{\Rpp}{\R_{>0}}
\newcommand{\Np}{\N_{>0}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Rx}{\mathbb{R}^{n_x}}
\newcommand{\Rp}{\mathbb{R}^{n_p}}
\newcommand{\Rn}{\mathbb{R}^{n}}
\newcommand{\Ru}{\mathbb{R}^{n_u}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\PPP}{\mathscr{Y}}
\newcommand{\F}{\mathcal{F}}
\newcommand{\J}{\mathcal{J}}
\newcommand{\CC}{\mathcal{C}}
\newcommand{\CCd}{\mathcal{C}^\delta}
\newcommand{\CCdinf}{\mathcal{C}^\delta}
\newcommand{\JC}{\J_{\CC}}
\newcommand{\jc}{J_{\CC}}
\newcommand{\jj}{J}
\renewcommand{\L}{\mathscr{L}}
\newcommand{\p}{\bar{p}}
\newcommand{\PP}{\mathscr{P}}
\newcommand{\mpc}{\mathrm{MPC}}
\newcommand{\tto}{\rightrightarrows}
\newcommand{\jct}{\ensuremath{J_{\CCd}}}
\renewcommand{\P}{\mathscr{P}}

\usepackage[dvipsnames]{xcolor}
\newcommand{\rz}[1]{#1}
\newcommand{\rzbegin}{\relax}
\newcommand{\rzend}{\relax}
% \newcommand{\rz}[1]{\textcolor{orange1}{#1}}
% \newcommand{\rzbegin}{\begingroup\color{orange1}}
% \newcommand{\rzend}{\endgroup}

% Add vertical lines in algorithms
\usepackage{tikz}
\usepackage{pgfplots}
\pgfplotsset{compat=newest}
\usepgfplotslibrary{groupplots}
\usepackage{hf-tikz}
\usetikzlibrary{tikzmark}
\usetikzlibrary{
    shapes.geometric, 
    positioning, 
    calc,
    arrows.meta
}

% customize captions
\usepackage[
    format=plain,
    justification=RaggedRight,
    labelfont={bf},
    font={small},
]{caption}
\captionsetup[table]{
    position=top,
    skip=5pt
}

% hyperlink colors
% \hypersetup{allcolors=blue4}
